CARD: Semantic Segmentation with Efficient Class-Aware Regularized Decoder

Semantic segmentation has recently achieved notable advances by exploiting "class-level" contextual information during learning. However, these approaches simply concatenate class-level information to pixel features to boost the pixel representation learning, which cannot fully utilize intra-class and inter-class contextual information. Moreover, these approaches learn soft class centers based on coarse mask prediction, which is prone to error accumulation. To better exploit class level information, we propose a universal Class-Aware Regularization (CAR) approach to optimize the intra-class variance and inter-class distance during feature learning, motivated by the fact that humans can recognize an object by itself no matter which other objects it appears with. Moreover, we design a dedicated decoder for CAR (CARD), which consists of a novel spatial token mixer and an upsampling module, to maximize its gain for existing baselines while being highly efficient in terms of computational cost. Specifically, CAR consists of three novel loss functions. The first loss function encourages more compact class representations within each class, the second directly maximizes the distance between different class centers, and the third further pushes the distance between inter-class centers and pixels. Furthermore, the class center in our approach is directly generated from ground truth instead of from the error-prone coarse prediction. CAR can be directly applied to most existing segmentation models during training, and can largely improve their accuracy at no additional inference overhead. Extensive experiments and ablation studies conducted on multiple benchmark datasets demonstrate that the proposed CAR can boost the accuracy of all baseline models by up to 2.23% mIOU with superior generalization ability. CARD outperforms SOTA approaches on multiple benchmarks with a highly efficient architecture.

==> old_SAA_section.tex <==
\subsubsection{Synced Axial Attention}
\label{sec:method:spatial-token-mixer}


\hy{The spatial token mixer~\cite{cMetaFormer} provides the context aggregation between each pixel's encoding.
%
Although we found that a regular self-attention~\cite{cNonLocal} as the decoder can perform very well with our proposed CAR, its computational cost in the spatial domain has an unacceptable computational cost, especially when the input data has a large resolution.
%
Years ago, many sparse replacement methods~\cite{cCCNet,cOCR,cCAA} already had a comparable performance with regular self-attention but with a much smaller computational cost.
%
However, in our experiments (see below Tab.~\ref{tab:CAR:AblationsBaseline}), methods like CCNet~\cite{cCCNet} show limited compatibility with our proposed CAR.
%
Yet their performance is improved, but less than CAR + regular self-attention (\textcolor{blue}{+0.56} vs \textcolor{blue}{+2.18} with ResNet-50)}


\hy{We also find recently proposed CAA~\cite{cCAA} shows relevantly better compatibility with our proposed CAR than other sparse self-attention approaches. 
%
Regrettably, it is an uncommon novel operation that has small FLOPs but has an actual slow speed in some hardware due to the lack of hardware and software (e.g, driver) support.}


\dknote{real method descriptions starts from here}
\hy{Thus, the goal of the spatial token mixer in our proposed CARD should have well compatibility with CAR that results in a good performance, a smaller computational cost than regular self-attention, and be supported by current hardware and software to have a comfortable speed. }

\hyna{
In CARD, we proposed an improved version of multi-head axial attention as the token mixer, named \saa (SAA).
%
As shown in Fig.~\ref{fig:CARD:SAA}a, column attention (vertical) and row attention (vertical) perform separately in Vanilla Axial Attention.
%
The proposed SAA is different, as shown in Fig.~\ref{fig:CARD:SAA}b. We only compute the query, key, and value once, and the same query and key are used to generate the column attention map and row attention map.
%
Also, after the column context aggregation is completed, the result is directly used to perform the context aggregation via row attention map without an extra `value' transformation.
%
Thus, SAA provided consistent feature space when compute the attention map for column and row, since they are generated by the same query and key.
%
The consistent feature space avoid the possible error accumulation in Vanilla Axial Attention where the row attention map is generated based on the column context aggregation result, which can include bias.
%
It is benefit for the global context aggregation, since the target of the spare attention is provide similar performance with regular self-attention with smaller computational cost.
%
It also brings a better compatibility with the proposed CAR, because the consistent feature space allows the CAR can perform the optimization in the global context prospective, just as the regular self-attention.
%
Thus, SAA fused the separated column and rowed attention in Vanilla Axial Attention, which not only brings smaller computational costs (without the extra linear convolutions for query, key, and value) but also brings improved performance and CAR friendly.
}


\hy{
Besides, in recent two years, many works have discussed the possible negative impact of positional encoding on semantic segmentation tasks, where the resolution sensitivity is a commonly acknowledged root cause.
%
\dknote{just say we use CPE, [add ref here]. then describe what is CPE.}
Thus, in our CARD, we use a similar design in~\cite{cCPvT,cMaxViT} for the positional encoding before applying the token mixer, where the depth-wise $3\times3$ convolution generates the positional encoding, which is generalized on adjustable inputs resolution for semantic segmentation. 
%
Note that we did not apply normalization as in~\cite{cMaxViT} since we find it is harmful to the accuracy.
%
Furthermore, we found stack multiple token mixer + CAR can get slightly more accuracy. We did not perform that in CARD because it is inefficient, given more computational cost and GPU memory usage with limited accuracy improvement (3 layers less than 0.5\% mIOU).
}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


